GRPO Training Dynamics for Small Language Models

Group Relative Policy Optimization (GRPO) has emerged as a memory-efficient reinforcement fine-tuning (RFT) technique for reasoning-intensive tasks. How- ever, GRPO training dynamics on small language models (SLMs) remain poorly understood, limiting its reliable adoption and reproducibility in open and resource- constrained environments. In this work, we present a systematic study of GRPO fine-tuning for SLMs ranging from 1.5B to 7B parameters under a practical single- node 8xA100 compute budget. Our study spans multiple model families and reasoning domains, including mathematics, coding, and multiple-choice question answering (MCQ) in science. Across these settings, we analyze how group size affects policy convergence, training stability, and downstream benchmark per- formance. We further characterize tensor-level update dynamics during GRPO training and investigate whether the choice of LoRA target modules and layers can improve the performance of GRPO-tuned models. While our initial GRPO-tuned models outperform their base counterparts on approximately 80% of mathematical benchmark evaluations, they demonstrate limited capability on MCQ and code reasoning tasks. Guided by our mechanistic evaluations, we refined our LoRA and reward-shaping configurations to improve performance in latter domains. These findings provide practical guidance for GRPO training for SLMs.

==> assets/tables/mcq-benchmarks/bigbenchhard_ood_eval.tex <==
\begin{table}[!ht]
    \centering
    \caption{BigBenchHard OOD evaluation of base models and finetuned models using pass@k metric(1000 questions from 4 subsets, 5 samples per question)}
    \label{tab:bbh}
    \begin{tabular}{|l|l|l|l|}
    \hline
        model\_label & pass\_at\_1\_pct & pass\_at\_3\_pct & pass\_at\_5\_pct \\ \hline
        DS-LLM-7B-Chat (base) & 30.82 & 51.17 & 60.7 \\ \hline
        DS-LLM-7B GRPO s3407 G4 & 31.14 & 48.25 & 55.4 \\ \hline
        DS-LLM-7B GRPO s42 G16 & 30.62 & 45.55 & 51.7 \\ \hline
        DS-LLM-7B GRPO s42 G4 & 31.1 & 47.65 & 54.9 \\ \hline
        DS-R1-Qwen-1.5B (base) & 40.76 & 69.43 & 80.2 \\ \hline
        DS-R1-Qwen-1.5B GRPO s42 G16 & 41.42 & 68.8 & 79.3 \\ \hline
        DS-R1-Qwen-1.5B GRPO s42 G4 & 41.88 & 69.02 & 78.6 \\ \hline
        Nemotron-4B (base) & 31.4 & 51.45 & 61.1 \\ \hline
        Nemotron-4B GRPO s3407 G16 & 29.82 & 42.89 & 49.0 \\ \hline
        Nemotron-4B GRPO s3407 G4 & 31.32 & 50.28 & 59.5 \\ \hline
        Nemotron-4B GRPO s42 G16 & 31.52 & 46.71 & 54.3 \\ \hline
        Nemotron-4B GRPO s42 G4 & 30.24 & 48.87 & 57.8 \\ \hline
    \end{tabular}
\end{table}
